Topology, dynamics, and control of an octopus-analog muscular hydrostat

Muscular hydrostats, such as octopus arms or elephant trunks, lack bones entirely, endowing them with exceptional dexterity and reconfigurability. Key to their unmatched ability to control nearly infinite degrees of freedom is the architecture into which muscle fibers are weaved. Their arrangement is, effectively, the instantiation of a sophisticated mechanical program that mediates, and likely facilitates, the control and realization of complex, dynamic morphological reconfigurations. Here, by combining medical imaging, biomechanical data, live behavioral experiments and numerical simulations, we synthesize a model octopus arm entailing ~200 continuous muscles groups, and begin to unravel its complexity. We show how 3D arm motions can be understood in terms of storage, transport, and conversion of topological quantities, effected by simple muscle activation templates. These, in turn, can be composed into higher-level control strategies that, compounded by the arm's compliance, are demonstrated in a range of object manipulation tasks rendered additionally challenging by the need to appropriately align suckers, to sense and grasp. Overall, our work exposes broad design and algorithmic principles pertinent to muscular hydrostats, robotics, and dynamics, while significantly advancing our ability to model muscular structures from medical imaging, with potential implications for human health and care.

==> 03_methods.tex <==
\section*{Methods}
\textbf{Animal care and imaging.} 
Three adult female wild-caught \textit{O. rubescens} were used in this study: one for histology imaging, one for MRI imaging, and one for behavioral experiments. They were collected by Monterey Abalone, Inc. by trapping and shipped overnight to the University of Illinois in Urbana, IL. Animals were housed individually in temperature controlled (12 $^\circ$C) glass aquaria enriched with clay-pot dens and fed a steady diet of diced squid. All animal procedures were in compliance with ARRIVE guidelines regulating animal experimentation. 
All efforts were made to minimize animal suffering and to reduce the number of animals used. 

For imaging, two octopuses were anesthetized in seawater with 333 nM MgCl$_2$ concentration. An arm was amputated from each. All procedures carried out complied with institutional recommendations for cephalopods. After surgery and recovery from anesthesia, live animals were replaced in their recirculating cold-water tanks (12 $^\circ$C). The animals were monitored for signs of stress while left for healing. Animals accepted food at 2 days post-surgery and continued recovering well. The ex vivo tissues were quickly placed in Tris-buffered sea water bath (18 $^\circ$C) for experimental procedures. Arms were fixed in 4\% PFA for 48 hours (4 $^\circ$C). For  histology imaging, the arm was segmented into blocks along the cross-sectional and frontal planes, sectioned, and stained with hematoxylin and eosin to reveal the anatomical organization of the muscle fibers. Slides were imaged using a Nanozoomer 2.0-HT Slide Scanner.

For MRI imaging, the amputated arm was transferred to a 1x PBS solution and 24 hours prior to imaging the arm was placed in a tube with 15 mL of PBS and a 4 $\mu$L/mL gadolinium concentration. T2-weighted and DTI scans were performed with a 9.4T Brucker preclinical scanner and a surface receive coil. Slice direction was aligned with the arm’s axial orientation. For T2-weighted scans, a TURBO RARE sequence was acquired over a 20 mm FOV with a 256x256 matrix (78.125 $\mu$m in-plane resolution), 20 slices (1 mm thickness), and TE/TR=32/2500 ms. DTI scans were acquired for a 128x128 matrix (156.25 $\mu$m resolution), 20 slices (1 mm thickness), TE/TR = 32/1500 ms, 4 segments, 3 b-values of 500, 1000, and 1500 mm$^2$/s, 12 directions, and 16 averages. Fiber tractography was performed using DSI Studio \cite{Yeh:2013} over an ROI manually defined to isolate the arm.

\vspace{5pt}
\textbf{Arm behavior characterization from video recordings.} To characterize the modes of deformations employed by an octopus arm when manipulating objects, multiple trials of an \textit{O. rubescens} interacting with objects were filmed.
To isolate arm behaviors for recording, the octopus was placed in a clear acrylic box with a 3/8 inch diameter hole in the lower corner (sized to allow only 1-2 arms to reach through). 
Two objects of different shapes were presented outside the box near the hole and the octopus was allowed to freely reach through the hole and interact with them. A description of the objects used is provided in the SI. 
% During all trials, the operator was shielded from the octopus's view. 
Videos were recorded using a Sony Alpha a7III camera with an adjustable 18-135mm f/3.5-5.6 lens at 30 fps with either 1080p or 4k resolution. 
Trials were performed over several days until 23 independent interactions with each object were acquired.  
Videos were trimmed to isolate periods over which the arm was observed to interact with the object, and individual frames were extracted every 5 seconds, resulting in 691 total frames for analysis. 
% While the compliant interaction of the arm with the object and the adherence of the arm's suckers to the object will no doubt strongly influence the configuration of the arm, here we restrict ourselves to considering only the shape of the arm and not how the object or suckers might be influencing it. 
To quantify the deformation modes that emerge from the combination of muscular actuation, sucker adhesion, and environmental interactions, the shape of the arm was characterized based on the static poses visible in these frames.
Adopting a scoring methodology similar to that of Kennedy et al. \cite{Kennedy:2020} and Grasso \cite{Grasso:2008}, we considered deformations over the proximal, medial, and distal sections of the arm.  
For each section, the arm's pose was categorized as one-dimensional (straight), two-dimensional (planar bending or coiling), or three-dimensional (helical or multi-plane bending).
A detailed description of the categorization protocol and additional analysis is provided in the SI. 
Example clips of the acquired videos are available in \add{SI Video~1}.

\vspace{5pt}
\textbf{Modeling of an octopus arm.} We model the octopus arm as an assembly of Cosserat rods, which are slender, one-dimensional elastic structures that can undergo all modes of deformation: bending, twisting, stretching, and shearing. Representing an octopus arm's different muscle groups as Cosserat rods entails a number of advantages as, assembled together, they naturally capture the heterogeneity of muscular architectures. Further, the Cosserat formulation can be extended to account for non-linear material properties, connectivity, active stresses, internal pressure, and environmental loads. The numerical implementation of Cosserat rods is computationally efficient as they accurately capture large deformations in 3D space through a one-dimensional representation, alleviating time-consuming meshing difficulties and compute costs of 3D elasticity.

\vspace{5pt}
\textit{\uline{Dynamics of a single Cosserat rod.}} An individual Cosserat rod is described by its center line position $\mathbf{\bar{x}}(s,t) \in \mathbb{R}^{3}$ and an oriented reference frame of (row-wise) orthonormal directors $\mathbf{Q}(s,t) \in \mathbb{R}^{3 \times 3} =\left[\mathbf{\bar{d}}_{1}, \mathbf{\bar{d}}_{2}, \mathbf{\bar{d}}_{3}\right]^{-1}$ along its length $s \in [0, L(t)]$, where $L(t)$ is the current length, for all time $t \in \mathbb{R} \ge 0$ (Fig.~\ref{fig:cosserat_rod_model}). 
Any vector defined in the global \textit{lab frame} ($\mathbf{\bar{v}}$) can be transformed into the \textit{local frame} ($\mathbf{{v}}$) via $\mathbf{v} = \mathbf{Q}\mathbf{\bar{v}}$ and from the local to the lab frame via $\mathbf{\bar{v}} = \mathbf{Q}^{T}\mathbf{v} $. 
For an unshearable and inextensible rod, $\mathbf{\bar{d}}_{3}$ is parallel to the rod's local tangent ($\partial_s \mathbf{\bar{x}} = \mathbf{\bar{x}}_{s}$), and 
 $\mathbf{\bar{d}}_{1}$ (normal) and $\mathbf{\bar{d}}_{2}$ (binormal) span the rod's cross-section.
However, under shear or extension, the rod's tangent direction $\mathbf{\bar{x}}_{s}$ and $\mathbf{\bar{d}}_{3}$ are no longer the same, with the difference represented by the shear strain vector $\bm{\epsilon} = \mathbf{Q} \left(\mathbf{\bar{x}}_{s} -  \mathbf{\bar{d}}_{3} \right)$. 
The gradient of the directors ($\mathbf{\bar{d}}_j$) with respect to the rod's length is defined by the curvature vector $\bm{\bar{\kappa}}(s,t) \in \mathbb{R}^{3}$ through the relation $\partial_s \mathbf{\bar{d}}_{j} = \bm{\bar{\kappa}} \times \mathbf{\bar{d}}_{j}$. In the local frame ($\bm{\kappa} = \mathbf{Q} \bm{\bar{\kappa}}$), the components of the curvature vector $\bm{\kappa} = [\kappa_1,~\kappa_2,~\kappa_3]$ relate to bending (${\kappa}_{1}$ and ${\kappa}_{2}$) and twisting (${\kappa}_{3}$) of the rod.
Similarly, the gradient of the directors with respect to time is defined by the angular velocity vector $\bm{\bar{\omega}}(s,t) \in \mathbb{R}^{3}$ through the relation $\partial_t \mathbf{\bar{d}}_{j} = \bm{\bar{\omega}} \times \mathbf{\bar{d}}_{j}$. The linear velocity of the centerline is $\mathbf{\bar{v}}(s,t) \in \mathbb{R}^{3}=\partial_t \mathbf{\bar{x}}$ while the second area moment of inertia $\mathbf{I}(s,t)\in \mathbb{R}^{3 \times 3}$, cross-sectional area ${A}(s,t)\in \mathbb{R}$, and density $\rho(s)\in \mathbb{R}$ are defined based on the rod's material properties.
The dynamics of a Cosserat rod are then described as\cite{Gazzola:2018} 
% \begin{equation} 
%     \partial_{t}^{2} \left( \rho A \mathbf{\bar{x}} \right) = \partial_s \left(\frac{\mathbf{Q}^{T} \mathbf{n} }{e}
%     \right) + e \mathbf{\bar{f}}
%     \label{eqn:linear_momentum}
% \end{equation}
\begin{equation} 
    \partial_{t}^{2} \left( \rho A \mathbf{\bar{x}} \right)= \partial_s \left(\mathbf{Q}^{T} \mathbf{n}\right) + \mathbf{\bar{f}}
    \label{eqn:linear_momentum}
\end{equation}
% 
% \begin{equation}\label{eqn:angular_momentum}
%     \begin{split}
%     \frac{\rho \mathbf{I}}{e} \cdot \partial_t \bm{\omega} &= \partial_s \left(\frac{\bm{\tau}}{e^3}\right)
%     +\frac{\bm{\kappa} \times \bm{\tau}}{e^3} 
%     + \left( \mathbf{Q} \frac{\mathbf{\bar{x}}_s}{e} \times \mathbf{n} \right) \\
%         & + \left(\rho \mathbf{I} \cdot \frac{\mathbf{\omega}}{e}\right)\times \mathbf{\omega} 
%         + \frac{\rho \mathbf{I} \mathbf{\omega}}{e^2} \cdot \partial_t e + e \mathbf{c}\\
%     \end{split}
% \end{equation}
\begin{equation}\label{eqn:angular_momentum}
    \partial_t \left( \rho \mathbf{{I}} \bm{{\omega}} \right) = \partial_s \bm{{\tau}} + \bm{\kappa} \times \bm{\tau} + \left(\mathbf{Q} \mathbf{\bar{x}}_s \times \mathbf{n}\right)
     + \left(\rho \mathbf{I} \bm{\omega}\right) \times \mathbf{\omega} +  \mathbf{Q}\mathbf{\bar{c}}
\end{equation}
where Eq.~\ref{eqn:linear_momentum} (lab frame) and  Eq.~\ref{eqn:angular_momentum} (local frame) represent the linear and angular momentum balance at every cross-section, respectively,
% $e=\left| \mathbf{\bar{x}}_s\right|$ is the local stretching factor, 
$\mathbf{n}(s,t)\in \mathbb{R}^{3}$ and $\bm{\tau}(s,t)\in \mathbb{R}^{3}$ are internal forces and couples, respectively,  developed due to elastic deformations and muscle contractions while $\mathbf{\bar{f}}(s,t)\in \mathbb{R}^{3}$ and $\mathbf{\bar{c}}(s,t)\in \mathbb{R}^{3}$ capture external forces and couples applied to the arm, respectively.

For a linear elastic material, the internal forces $\mathbf{{n}} = [n_1,~n_2,~n_3]$ are proportional to the shear strain of the rod $\mathbf{{n}} = \mathbf{{S}} \left(\bm{\epsilon} - \bm{\epsilon}_0 \right)$ where $\bm{\epsilon}_0$ is the intrinsic shear strain of the rod, $\mathbf{S} = \text{diag}\left(\alpha_c G A, ~\alpha_c G A, ~E A \right)$ is the rod's shear/stretch stiffness matrix, $E$ is the rod's Young's modulus, $G$ is the rod's shear modulus, and $\alpha_c$ is the Timoshenko shear correction factor\cite{Gazzola:2018}.
Octopus muscles, however, exhibit non-linear elastic properties in both their passive response to stretch and their ability to actively generate force. To account for this material behavior, we directly modify the axial stretch component ($n_3$) of the internal force vector $\mathbf{n}$ (described in the next section) while modeling its shear components ($n_1$, $n_2$) using the above presented linear elastic formulation. We additionally model internal elastic torques $\bm{\tau}$ using the linear relationship $\bm{\tau} = \mathbf{B} \left(\bm{\kappa} - \bm{\kappa}_0 \right)$
where $\bm{\kappa}_0$ is the intrinsic curvature of the rod, $\mathbf{B} \in \mathbb{R}^{3 \times 3}  = \text{diag}\left(E {I}_1, ~E {I}_2, ~G {I}_3 \right)$ is the rod's bend/twist stiffness matrix, and ${I}_{1}$, ${I}_{2}$, and ${I}_{3}$ are the rod's second moments of inertia about $\mathbf{\bar{d}}_1$, $\mathbf{\bar{d}}_2$, and $\mathbf{\bar{d}}_{3}$, respectively. Material and geometric properties for the different muscle groups are based on experimental measurements and are provided in the SI. 

The above continuous representation is discretized into $\left(n_{\text{elem}}+1\right)$ nodes of position $\mathbf{\bar{x}}_{i}$ that are connected by $n_{\text{elem}}$ cylindrical elements. Linear displacements are determined by the internal and external forces acting at the nodes, while rotations are accounted for via couples applied to the cylindrical elements. 
The dynamic behavior of a rod is computed by integrating the discretized set of equations, along with appropriate boundary conditions, in time via a second-order position Verlet scheme\cite{Gazzola:2018}. 
Energy losses due to internal friction and viscoelastic effects are captured using a combination of Rayleigh potentials and Laplacian filters (described in the SI). 
This numerical approach has been validated against a number of benchmark problems with known analytic solutions as well as experimental investigations involving contact, anisotropic surface friction, and highly viscous fluids\cite{Gazzola:2018}. In this study, we used PyElastica\cite{PyElastica}, which is an open-source, Python-based implementation of this numerical scheme and has previously been demonstrated in a number of engineering and biophysical contexts, from the design of soft and bio-hybrid robots \cite{Naughton:2021,Aydin:2019,Wang:2021} to the modeling of musculoskeletal architectures, including snakes \cite{Zhang:2021} and human biceps \cite{Zhang:2019}.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/cosserat_rod_figure_v3-light-01}
    \caption{
    % \textcolor{red}{[NN notes: 1) move $\mathbf{\bar{x}}_s$ left to be in whitespace 2) change $\mathbf{c}$ to $\mathbf{\bar{c}}$ 3) make shear vector arrow thicker (actually, make all arrows thicker) 4) Maybe move Q to upper right corner? We should fill that space. ]}
    \textbf{Cosserat rod model}: A Cosserat rod in three-dimensional space is described by a centerline $\mathbf{\bar{x}}(s,t)$ and a local frame $\mathbf{Q}(s,t)=\left[\mathbf{\bar{d}}_{1}, \mathbf{\bar{d}}_{2}, \mathbf{\bar{d}}_{3}\right]^{-1}$. Both are functions of rod's arc-length $s$ and time $t$. 
    % The orange and purple lines trace out $\bar{\mathbf{d}}_{1}(s,t)$ and $-\bar{\mathbf{d}}_{1}(s,t)$, respectively.
    % In the case of extension or compression the current filament arc-length $s$ is different than the rest reference arc-length $\hat{s}$ and this is captured by scalar dilatation field $e$.
    % Current total length of filament is shown as $L(t)$. 
    The shear vector $\bm{\epsilon}$ quantifies the deviation of  $\bar{\mathbf{d}}_{3}(s,t)$ from the rod's tangent $\bar{\mathbf{x}}_{s}(s,t)$.
    External forces and couples that deform the elastic rod are denoted as $\bar{\mathbf{f}}(s,t)$ and  $\bar{\mathbf{c}}(s,t)$ respectively.
    Yellow and pink lines trace out the orientation of $\bar{\mathbf{d}}_{1}(s,t)$ and $-\bar{\mathbf{d}}_{1}(s,t)$ along the rod, respectively. 
    }
    \vspace{-20pt}
    \label{fig:cosserat_rod_model}
\end{figure}



\vspace{5pt}
\textit{\uline{Modeling the active and passive mechanics of octopus muscles.}}\label{sec:muscle_model} Biological muscles actively generate internal forces that cause them to axially contract while simultaneously exhibiting hyperelastic passive behavior when stretched. Both effects render a linear elastic treatment of the Cosserat rod's axial stretch inaccurate in the context of the octopus. Instead, we model the axial component ($n_3$) of the internal force vector $\mathbf{n}$ by considering the active $\sigma_{a}(s,t) \in \mathbb{R}$ and passive $\sigma_{p}(s,t) \in \mathbb{R}$ axial stresses developed along each muscle
\begin{equation}
n_3 = A (\sigma_a + \sigma_p)
\end{equation}
The active stresses developed by the muscle are modeled as \cite{VanLeeuwen:1997}
\begin{equation}\label{eqn:non_linear_muscle_model}
    \sigma_{a} = f_{a} \sigma_{\max} f_{l} f_{v} 
\end{equation}
where $f_{a}(s,t) \in [0,1]$ is the muscle's activation level,  $\sigma_{\max}$ is the maximum stress the muscle can develop, and
$f_{l}$ and $f_{v}$ capture, respectively, the force-length and force-velocity dependence at play during muscle contractions. Note that $f_{a}(s,t)$ can spatially vary along the rod's length $s$.


Zullo and coworkers \cite{zullo2022octopus} have previously experimentally characterized the active and passive mechanical properties of \textit{Octopus vulgaris} longitudinal and transverse muscles. Their reported experimental data were digitized (details in SI) and used to determine active and passive material properties of both the longitudinal and transverse muscle groups. 
For each muscle group, an $8^{\text{th}}$-order polynomial was fit to the digitized data to determine the active force-length relationships as a function of axial strain 
\begin{equation}
    f_{l} = \sum_{i=0}^{8} a_{i} \left(\epsilon+1 \right)^{i}
\end{equation}
where $a_i$ are the polynomial coefficients and $\epsilon= \bm{\epsilon} \cdot \mathbf{Q}\mathbf{\bar{d}}_3$ is the axial strain.
Numerical values of $a_i$ are reported in Supplementary Table 1.
Additionally, based on the reported data, we set $\sigma_{\max}=130$ kPa for all muscle groups. Experimental data of the force-velocity relationship $f_v$ of octopus muscle has not yet been reported so we model this dependence as a function of strain rate $\dot{\epsilon} = \partial_t \epsilon$ using a relationship previously reported by Van Leeuwen and Kier\cite{VanLeeuwen:1997} for the transverse muscles of squid tentacle muscles 
\begin{equation}
    f_v = 
        \begin{cases}
        1.8 - 0.8 \frac{1+\dot{\epsilon}^{*}}{1 - 7.56 \dot{\epsilon}^{*} / 0.25} \quad \text{for } \dot{\epsilon}^{*} < 0\\
        \frac{1 - \dot{\epsilon}^{*}}{1 + \dot{\epsilon}^{*}/0.25} \hspace{48pt} \text{for } \dot{\epsilon}^{*} \ge 0
        \end{cases}
\end{equation}
where  $\dot{\epsilon}^{*}= \dot{\epsilon}/\dot{\epsilon}_{\min}$ and $\dot{\epsilon}_{\min} = -1.8$ is the minimum strain rate\cite{VanLeeuwen:1997}. This relation was experimentally validated against experimental recordings of squid tentacle strikes \cite{Kier:1997} and we further characterized the accuracy of our overall approach against the same experiments (see SI).

Passive force-length behaviors are similarly determined by fitting an $8^{\text{th}}$-order polynomial to the digitized experimental data of Zullo et al. \cite{zullo2022octopus} longitudinal and transverse muscle's passive response under axial stretch. We supplement this with a linear elastic model of muscle's response under compression, resulting in the overall passive response 
\begin{equation}
        \sigma_{{p}} = 
        \begin{cases}
        \sigma_{\max} \sum_{i=0}^{8} b_{i} \left(\epsilon+1 \right)^{i}   \quad \text{ for } \epsilon >0\\
        E_{{c}} \epsilon \hspace{62pt} \text{ for } \epsilon \le 0
        \end{cases}
\end{equation}
Numerical values of $b_i$ are reported in Supplementary Table 2.
The Young's modulus under compression $E_{{c}}$ is set consistent with indentation stiffness measurements of \textit{O. vulgaris} suckers\cite{Tramacere2014} (25 kPa for longitudinal and oblique muscles and 10 kPa for transverse muscles).

To control individual muscle groups, we utilize three activation templates: a ramp-up activation over either a localized interval or globally over the entire muscle group, an activation wave that travels along the arm, and a sigmoid wavefront that travels outward from the arm's base. Additional details on the templates are provided in the SI. 

\vspace{5pt}
\textit{\uline{Assembling Cosserat rods into an octopus arm.}}\label{sec:connections} We assemble our octopus arm by arranging active and passive rods into a representative muscular architecture based on medical imaging. The arm in its rest configuration presents no muscle activation or residual stresses. A description of the arm's geometry and parameters used is provided in the SI. 
To fix the base of the arm in place, zero-displacement boundary conditions are defined at the nodes of the LM and ANC nearest to the base.  
We also define three classes of boundary conditions 
that together capture the possible modes of interaction between neighboring rods. This mechanical connectivity enables the arm to translate the one-dimensional internal contraction forces generated by individual muscles into the three-dimensional dynamic motions of the arm as a whole. As a general strategy, 
we enforce `soft' interaction constraints through displacement-force (or torque) correction relationships \cite{Zhang:2019}. 

\vspace{5pt}
\textit{\uline{Connecting rods via distributed boundary conditions.}} To connect neighboring rods together, we implement a distributed displacement-force boundary condition to capture, at first-order, the response of the collagen connective tissue that surrounds and binds together the octopus' muscle groups\cite{Kier:2007}. Details of how connections are geometrically defined vary depending on the specific muscle groups being connected and are provided in the SI. However, the general mechanical approach is similar for all groups. 
Given two neighboring elements $R_i$ for $i\in\{1,2\}$ belonging to two rods that are to be connected, we define a force-displacement boundary condition proportional to the distance between their corresponding locations on the surface of each rod $\mathbf{\bar{x}}^{s}_{i}=\mathbf{\bar{x}}^{c}_{i}+r_{i} \mathbf{\bar{s}}_{i}$, where $\mathbf{\bar{x}}^{c}_{i}$ denotes the center position of elements $R_i$, and $r_{i}$ is the element's radius. 
The unit vector $\mathbf{\bar{s}}_{i}$ denotes the point on the surface of $R_i$ where the connection is located. It is defined in the rest configuration such that $\mathbf{\bar{s}}_{1}$ points from $\mathbf{\bar{x}}^{c}_{1}$  to $\mathbf{\bar{x}}^{c}_{2}$ and $\mathbf{\bar{s}}_{2} = -\mathbf{\bar{s}}_{1}$.
Then, at each timestep, a restoring force and torque proportional to the distance between these two points $\bm{\bar{\delta}}^{s}_{i}=\mathbf{\bar{x}}^{s}_{j} - \mathbf{\bar{x}}^{s}_{i}$ for $i\in\{1,2\}$ and $j\in\{2,1\}$ is applied as an external force and couple to each element 
\begin{equation}
    \begin{aligned}
    \mathbf{\bar{F}}_{i} &= \alpha_{s} k_{s} \bm{\bar{\delta}}_{i}^{s}\\
    \mathbf{\bar{C}}_{i} &= r_{i} \mathbf{\bar{s}}_{i} \times \mathbf{\bar{F}}_{i} 
    \end{aligned} \quad \forall i\in\{1,2\}
\end{equation}
where $\alpha_{s}$ is a scaling parameter and $k_{s}$ is a spring constant that is a function of the material and geometric properties of the rods. 
Dissipative effects related to the connective tissue's viscoelastic material response are implicitly accounted for at the level of our overall integration scheme through the use of Rayleigh potentials and Laplacian filters (described in the SI). 

% This captures elastic restoring effects. 
% Dissipative effects related to the viscous material response are consistently applied to all tissue elements (rods and connections) at the level of our overall integration scheme, using a combination of Rayleigh potentials and Laplacian filters (described in the SI). 


\vspace{5pt}
\textit{\uline{Contact between rods.}}\label{sec:contact_btw_rods} In addition to connecting rods together, we consider the forces that arise from contact between two elements $R_i$ for $i\in\{1,2\}$.
We consider contact to occur when $\epsilon_{i} \ge 0$ for $\epsilon_{i}=r_{i}+r_{j}-|\bm{\delta}^{c}_{i}|$ where $\bm{\delta}^{c}_{i}=\bar{\mathbf{x}}^{c}_{j}-\bar{\mathbf{x}}^{c}_{i}$ is the distance vector between the center location of the elements for $i\in\{1,2\}$ and $j\in\{2,1\}$.
We model contact between these two elements as a repulsive force $\bar{\mathbf{F}}_{i}$ on element $R_i$ based on the Hertzian contact model\cite{Hertz:1882}
\begin{equation}
    \bar{\mathbf{F}}_{i}= -H(\epsilon_{i}) \alpha_c k_{c} \epsilon_{i}^{3/2} \hat{\bm{\delta}}^{c}_{i} \quad \forall i\in\{1,2\}
\end{equation}
where $H(\cdot)$ is a Heaviside function that ensures a force is produced only in case of contact $\left(\epsilon_{i} \ge 0 \right)$, $\hat{\bm{\delta}}^{c}_{i}=\bm{\delta}^{c}_{i}/|\bm{\delta}^{c}_{i}|$, $\alpha_c$ is a scaling parameter, and $k_c$ is the contact stiffness coefficient which is a function of the material and geometric properties of the rods and is defined in the SI. This (soft) approach allows some amount of penetration to occur during arm deformations, quantification of the degree of penetration (Supplementary Fig. 4) shows it to be small ($\epsilon_{i}/(r_{i}+r_{j}) \lesssim 0.15$), so that geometric architecture of the arm is never compromised, i.e. no rods slip past each other. 
% that geometric distortions do not occur. 
% \textcolor{red}{[What determines an acceptable range? Can we define it succinctly?]}\textcolor{blue}{Unless rod centers does not run pass each other. We define penetration strain function $\epsilon_{p} = -\epsilon_{ij}/(r_{i}+r_{j})$ between rod $R_{1}$ and $R_{2}$ elements. 
% In the case if $-1 \ll \epsilon_{p}<0$ then rod elements penetrate acceptable amount; $\epsilon_{p} \le -1$ is considered unacceptable. But we never come close to this point, ever observed maximum is $\epsilon_{p}=-0.3$}.

\vspace{5pt}
\textit{\uline{Intramuscular pressure.}} A key mode of deformation for muscular hydrostats is the exploitation of muscle's near incompressibility to convert radially compressive stresses into axial elongation. In the octopus, this is achieved by contracting the transverse muscles to squeeze the arm and thus extend it. We incorporate this intramuscular pressure effect into our Cosserat rod formulation by computing a resultant radial stress, which we define as the magnitude of the external contact force vectors that cancel out with the components of contact force vectors in opposite directions. We translate this radial compression stress into an axial elongation stress by treating the element as a linearly isotropic and incompressible elastic rod so that $\sigma_{a}=-\sigma_{r}$. This axial extension stress is scaled by the element's cross-sectional area and applied as an external force along the elements axis $\mathbf{\bar{F}}_{a} = -A_{c} \sigma_{r} \mathbf{\bar{d}}_3$. Details of the exact procedure for computing the resultant radial compression stress are provided in the SI. 

\vspace{5pt}
\textbf{Environmental interactions.} We consider two forms of interactions: contact with external solid object and fluid drag.

\vspace{5pt}
\textit{\uline{Rigid body contact.}} All external obstacles are modeled as fixed, rigid cylinders discretized into elements along its axial length. We model their interaction with the arm through a combination of friction and contact boundary conditions applied to the outermost muscle fibers (oblique muscles), following the approach of Haff and Werner\cite{Haff:1986}. Similar to contact between neighboring rods, we define contact between a rod element $R_i$ and a cylinder element $C_j$ as occurring when $\epsilon_{i} \ge 0$ for $\epsilon_{i}= r_{i} + r_{j} - |\bm{\delta}^{c}_{i}|$, where $r_i$ and $r_j$ are the radii of the element and obstacle, respectively, and $\bm{\delta}^{c}_{i} = \mathbf{x}^c_{j} - \mathbf{x}^c_{i}$ is the distance between the center-points of rod element $R_{i}$ and the nearest element of the obstacle $C_{j}$. We model both repulsive and energy-dissipative forces that arise during contact via a contact (normal) force term
\begin{equation}
    \bar{\mathbf{F}}^{r}_{i} = H(\epsilon_{i}) \left(-k_{r} \epsilon_{i} - \gamma_r \bar{\mathbf{v}}_{i} \cdot \hat{\bm{\delta}}^{c}_{i} \right) \hat{\bm{\delta}}^{c}_{i}
\end{equation}
where $H(\cdot)$ is the Heaviside function, $\hat{\bm{\delta}}^{c}_{i} =\bm{\delta}^{c}_{i}/|\bm{\delta}^{c}_{i}| $, and $\bar{\mathbf{v}}_{i} = \bar{\mathbf{v}}_{j} - \bar{\mathbf{v}}_{i}$ is the relative velocity of the rod element and the obstacle element.
The penetration distance $\epsilon_{i}$ is scaled by the coefficient $k_r$ to compute the restoring force, which is then modulated by an energy dissipation term proportional to the coefficient $\gamma_r$ and the normal component of the relative velocity $\bar{\mathbf{v}}_{i} \cdot \hat{\bm{\delta}}^{c}_{i}$.
We model friction (shear) effects along the contacting surface of the arm and the obstacle according to 
% the model proposed by Haff and Werner\cite{Haff:1986}
% we model the effects of both static and kinetic friction as 
\begin{equation}
    \bar{\mathbf{F}}^{f}_{i} = - \min(\gamma_f | \bar{\bf{v}}^s_{i} |, ~  \mu_f |\bar{\mathbf{F}}_i^r |) \frac{\bar{\mathbf{v}}^s_{i}}{|\bar{\mathbf{v}}^s_{i}|}
\end{equation}
where  $\bar{\mathbf{v}}^s_{i} = \bar{\mathbf{v}}_{i} - \left(\bar{\mathbf{v}}_{i} \cdot \hat{\bm{\delta}}^{c}_{i} \right)\hat{\bm{\delta}}^{c}_{i}$ is the surface slip velocity between the rod and cylinder, $\mu_f$ is the Coulomb friction coefficient, and $\gamma_f$ is a friction damping coefficient. 
Values of $k_r$, $\gamma_r$, $\mu_f$ and $\gamma_f$ are given in Supplementary Table 4.


\vspace{5pt}
\textit{\uline{Fluid drag on the arm.}}\label{sec:drag_model} Drag forces depend on the geometrical and surface properties of the arm as well as fluid properties and flow conditions. 
While the full resolution of hydrodynamic effects is beyond the scope of this paper, we do implement a simplified drag model. This is based on the assumption that, within the octopus' operational regime, relevant time and length scales allow us to consider the flow environment as inertia-dominated. Under this assumption, drag may be modeled as proportional to the density of water $\rho_w$, the square of the arm's velocity $\mathbf{v}$, and the surface area perpendicular to the flow. Specifically, we model drag forces in the perpendicular $\bar{\mathbf{F}}^{D}_{p}$ and tangential $\bar{\mathbf{F}}^{D}_{t}$ direction of the arm using the approach first proposed by Yekutieli et al.\cite{Yekutieli:2005-1}
\begin{equation}\label{eqn:drag_formula}
    \begin{aligned}
        \bar{\mathbf{F}}^{D}_{t} &= -0.5 \rho_{w} A_{t} C_{t} |\bar{\mathbf{v}}_{t}|^2 {\bm{\eta}}_{t} \\
        \bar{\mathbf{F}}^{D}_{p} &= -0.5 \rho_{w} A_{p} C_{p} |\bar{\mathbf{v}}_{p}|^2 {\bm{\eta}}_{p}\\
    \end{aligned}
\end{equation}
where $A_{t}=2\pi r l$ is the arm's surface area, $A_{p}=2 r l$ is the arm's projected area in the perpendicular direction, $\bar{\mathbf{v}}_{t}=\left(\bar{\mathbf{v}} \cdot \bar{\mathbf{x}}_{s}\right)\bar{\mathbf{x}}_{s}$ and $\bar{\mathbf{v}}_{p}=\left(\bar{\mathbf{v}}- \bar{\mathbf{v}}_{t} \right)$ are the arm's velocities in the tangential and perpendicular directions, respectively, 
% \textcolor{red}{$\bar{\mathbf{v}}_{t}=\left(\bar{\mathbf{v}} \cdot \bar{\mathbf{x}}_{s}\right)\bar{\mathbf{x}}_{s}$ and $\bar{\mathbf{v}}_{p}=\left(\bar{\mathbf{v}}- \bar{\mathbf{v}}_{t} \right)$ are the arm's velocities in the tangential and perpendicular directions, respectively,}
and ${\bm{\eta}}_{t} = \bar{\mathbf{v}}_{t}/|\bar{\mathbf{v}}_{t}|$ and ${\bm{\eta}}_{p} = \bar{\mathbf{v}}_{p}/|\bar{\mathbf{v}}_{p}|$ are the normalized velocity directions. 
Here, $C_{t}=0.0256$ and $C_{p}=1.01$ are experimentally measured tangential and perpendicular drag coefficients of an \textit{O. vulgaris} arm \cite{Yekutieli:2005-1}.
% \strike{while $C_{p}=1.1$ is the drag coefficient of cross-flow over a rough cylinder at Re=912\cite{White:2006}.}
% for a cylinder under cross-flow at $Re=912$ \cite{White:2006}. 
% For numerical stability, drag forces are applied as external forces to the longitudinal muscles.
% both surface area $A_s$ and projected area $A_{p}$ are scaled according to the arm area.

\vspace{5pt}
\textbf{Knot theory calculations.} We compute link $\link$, writhe $\writhe$, and twist $\twist$ of the octopus arm according to the methodology developed by Charles et. al. \cite{Charles:2019} for knot theory calculations of open curves. This work showed that, while the Calugareanu-Fuller-White (CFW) theorem formally applies only to closed ribbons, if one extends the ends of an open curve outward, the CFW theorem holds to vanishingly small errors.
We consider the arm as a discretized, directed curve defined by the open axial curve $\bar{\mathbf{x}}_i(s,t)$ and an associated normal vector $\bar{\mathbf{d}}_{1,i}(s,t)$ based on the location and orientation of the axial nerve cord. 
% onto the normal-binormal plane of $\bar{\mathbf{x}}(s,t)$.
We extend this curve by appending straight, untwisted segments to the base and tip of the arm. At the base, the segment extends from $\bar{\mathbf{x}}_{0} + \alpha L \frac{\bar{\mathbf{x}}_{0} - \bar{\mathbf{x}}_{1}}{\left| \bar{\mathbf{x}}_{0} - \bar{\mathbf{x}}_{1} \right|}$  while at the tip the segment extends from $\bar{\mathbf{x}}_{n}$ to $\bar{\mathbf{x}}_{n} + \alpha L \frac{\bar{\mathbf{x}}_{n} - \bar{\mathbf{x}}_{n-1}}{\left| \bar{\mathbf{x}}_{n} - \bar{\mathbf{x}}_{n-1} \right|}$ where $\alpha >> 1$ and $L$ is the length of the rod.  
We empirically chose $\alpha=10^{3}$ to ensure deviation from the CFW was negligible ($ \left[\link - \left(\writhe + \twist \right) \right] \lesssim 10^{-6}$).
From this point, $\bar{\mathbf{x}}_i(s,t)$ will refer to this extended curve.
Finally, we define an auxiliary curve $\bar{\mathbf{r}}_i(s,t) = \bar{\mathbf{x}}_i(s,t) + r(s,t) \bar{\mathbf{d}}_{1,i}(s,t)$ where $r(s,t)$ is the local radius of the arm (yellow line in Fig.~\ref{fig:combined_primitives}b and Fig.~\ref{fig:cosserat_rod_model}; a  curve corresponding with $-\bar{\mathbf{d}}_{1}(s,t)$ is shown in pink). 
For these discretized curves, we compute link as 
\begin{equation}
    \link = \sum_{i=0}^{n+1} \sum_{j=0}^{n+1} \frac{1}{4\pi} \Omega_{i,j}
\end{equation}
where $\Omega_{i,j}$ is the solid angle determined by curves $\bar{\mathbf{x}}_i(s,t)$ and $\bar{\mathbf{r}}_j(s,t)$. 
The sum runs over $n+2$ for each curve, corresponding to $n$ physical segments and two additional segments. 
Similarly, since writhe is the link of the curve with itself, the same approach is used to compute writhe with the solid angle now $\Omega_{i,j}$ referring to the angle between two elements of curve $\bar{\mathbf{x}}_i(s,t)$ and $\bar{\mathbf{x}}_j(s,t)$.
Twist $(\twist)$ is the rotation of curve $\bar{\mathbf{r}}_i(s,t)$ around $\bar{\mathbf{x}}_i(s,t)$ and given as
\begin{equation}
    \twist = \frac{1}{2 \pi} \sum_{i=1}^{n-1} \phi_{i}
\end{equation}
where $\phi_{i}$ is the angle between $\bar{\mathbf{r}}_i(s,t)$ and $\bar{\mathbf{x}}_i(s,t)$ at each element $i$. 
See Section S2 of Charles et al. \cite{Charles:2019} for complete details. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/link-twist-writhe-figure-01.png}
%     \caption{
%     \textbf{Writhe-Twist}: A soft filament under different writhe and twist configurations.
%     }
%     \label{fig:writhe-twist-explanation}
% \end{figure}

